Depleted Fully Monolithic Active CMOS Pixel Sensors (DMAPS) in High Resistivity 150~nm Technology for LHC

Depleted monolithic CMOS active pixel sensors (DMAPS) have been developed in order to demonstrate their suitability as pixel detectors in the outer layers of a toroidal LHC apparatus inner tracker (ATLAS ITk) pixel detector in the high-luminosity large hadron collider (HL-LHC). Two prototypes have been fabricated using 150 nm CMOS technology on high resistivity (> 2 k$\Omega$ $cm^2$) wafers. The chip size is equivalent to that of the current ATLAS pixel detector readout chip. One of the prototypes is used for detailed characterization of the sensor and the analog readout of the DMAPS. The other is a fully monolithic DMAPS including fast readout digital logic that handles the required hit rate. In order to yield a strong homogeneous electric field within the sensor volume, thinning of the wafer was tested. The prototypes were irradiated with X-ray up to a total ionization dose (TID) of 50 Mrad and with neutrons up to non-ionizing energy loss (NIEL) of $10^{15}$ $n_{eq}/cm^2$. The analog readout circuitry maintained its performance after TID irradiation, and the hit-efficiency at > $10^7$ noise occupancy was as high as 98.9 % after NIEL irradiation.

==> mybibfile_short.tex <==
@techreport{atlas:letter,
    author        = {{ATLAS} Collaboration},
    title         = {Letter of Intent for the Phase-II Upgrade of the ATLAS Experiment},
    institution   = "CERN",
    address       = "Geneva",
    number        = "CERN-LHCC-2012-022. LHCC-I-023",
    year          = "2012",
    reportNumber  = "CERN-LHCC-2012-022",
}

@article{ivan:2007,
  title   = "A novel monolithic pixelated particle detector implemented in high-voltage {CMOS} technology",
  journal = {NIMA},
  volume  = "582",
  pages   = "876 -- 885",
  year    = "2007",
  author  = "I. Peric"
}

@article{ivan:2015,
    author={I. Peric and others},
    title={Overview of {HVCMOS} pixel sensors},
    journal={JINST},
    volume={10},
    number={05},
    pages={C05021},
    year={2015},
    abstract={High voltage CMOS (HVCMOS) sensors are presently considered for the use in Mu3e experiment, ATLAS and CLIC. These sensors can be implemented in commercial HVCMOS processes. HVCMOS sensors feature fast charge collection by drift and high radiation hardness. The sensor element is an n-well/p-type diode. This proceeding-paper gives an overview of HVCMOS projects and the recent results.}
}

@article{tianyang:2017,
    author={T. Wang and others},
    title={Development of a Depleted Monolithic {CMOS} Sensor in a 150 nm {CMOS} Technology for the {ATLAS} Inner Tracker Upgrade},
    journal={JINST},
    volume={12},
    number={01},
    pages={C01039},
    year={2017},
    abstract={The recent R&D focus on CMOS sensors with charge collection in a depleted zone has opened new perspectives for CMOS sensors as fast and radiation hard pixel devices. These sensors, labelled as depleted CMOS sensors (DMAPS), have already shown promising performance as feasible candidates for the ATLAS Inner Tracker (ITk) upgrade, possibly replacing the current passive sensors. A further step to exploit the potential of DMAPS is to investigate the suitability of equipping the outer layers of the ATLAS ITk upgrade with fully monolithic CMOS sensors. This paper presents the development of a depleted monolithic CMOS pixel sensor designed in the LFoundry 150 nm CMOS technology, with the focus on design details and simulation results.}
}

@article{irfu:2016,
    author={Y. Degerli and others},
    title={Pixel architectures in a {HV-CMOS} process for the {ATLAS} inner detector upgrade},
    journal={JINST},
    volume={11},
    number={12},
    pages={C12064},
    year={2016},
    abstract={In this paper, design details and simulation results of new pixel architectures designed in LFoundry 150 nm high voltage CMOS process in the framework of the ATLAS high luminosity inner detector upgrade are presented. These pixels can be connected to the FE-I4 readout chip via bump bonding or glue and some of them can also be tested without a readout chip. Negative high voltage is applied to the high resistivity (> 2 kΩ .cm) substrate in order to deplete the deep n-well charge collection diode, ensuring good charge collection and radiation hardness. In these pixels, the front-end has been implemented inside the diode using both NMOS and PMOS transistors. The pixel pitch is 50 μm × 250 μm for all pixels. These pixels have been implemented in a demonstrator chip called LFCPIX.}
}


@article{hirono:2015,
    title = "{CMOS} pixel sensors on high resistive substrate for high-rate, high-radiation environments",
    journal = "NIMA",
    volume = "831",
    pages = {94 -- 98},
    year = "2016",
    issn = "0168-9002",
    doi = "j.nima.2016.01.088",
    author = {Toko Hirono and others},
    keywords = "Pixel detector, CMOS sensor, MAPS, Active pixel sensor"
}

@INPROCEEDINGS{hirono:2016,
    author={Toko Hirono and others},
    booktitle={2016 IEEE NSS/MIC/RTSD},
    title={Characterization of fully depleted {CMOS} active pixel sensors on high resistivity substrates for use in a high radiation environment},
    year={2016},
    volume={},
    number={},
    pages={1--4},
    keywords={CMOS image sensors;CMOS integrated circuits;nuclear electronics;position sensitive particle detectors;radiation effects;radiation hardening (electronics);readout electronics;silicon radiation detectors;ATLAS High Luminosity Large Hadron Collider;CMOS process;DMAPS;fully depleted CMOS active pixel sensors;high-bias voltage;high-energy particle physics experiments;high-radiation environment;high-resistive sensor material;high-resistivity substrates;radiation hardness;readout chip;size 150.0 nm;total ionization dose;CMOS technology;Physics;Prototypes;Radiation effects;Sensors;Transistors;X-rays},
    doi= "10.1109/NSSMIC.2016.8069902",
    ISSN={},
    month={Oct},}

@Article{pdg:2016,
    title = {Review of Particle Physics},
    volume = {40},
    issn = {1674-1137},
    doi = {10.1088/1674-1137/40/10/100001},
    number = {10},
    urldate = {2018-01-08},
    journal = {Chinese Physics C},
    author = "{Particle Data Group} and Olive, K.A. and others",
    month = oct,
    year = {2016},
    pages = {100001},
}

@Article{tomasz:vertex,
    author =       {Hemperek, Tomasz},
    title =        "Overview and perspectives of depleted {CMOS} sensors",
    journal =      "Proc Sci",
    volume =       {submitted},
    year =         2018,
    eprint =       "",
    eprinttype =   "arxiv"
}

@article{kit,
    title = "Geant4 simulation of a filtered X-ray source for radiation damage studies",
    journal = "NIMA",
    volume = "675",
    pages = {118 -- 122},
    year = "2012",
    issn = "0168-9002",
    doi = {10.1016/j.nima.2012.01.029},
    author = {M. Guthoff and others},
    keywords = "X-ray, Energy spectrum, Silicon drift diode, Geant4"
}

@InProceedings{elsa:e3xd,
    author       = {N. Heurich and others},
    title        = {The New External Beamline for Detector Tests at {ELSA}},
    booktitle    = {Proc. of IPAC'16},
    pages        = {4088 -- 4090},
    paper        = {THPOY002},
    language     = {english},
    keywords     = {simulation, quadrupole, radiation, electron, detector},
    venue        = {Busan, Korea},
    number       = {7},
    month        = {June},
    year         = {2016},
    isbn         = {978-3-95450-147-2},
    doi          = {10.18429/JACoW-IPAC2016-THPOY00s2},
}

@article{jsi,
    title = "Computational analysis of irradiation facilities at the {JSI} {TRIGA} reactor",
    journal = "Applied Radiation and Isotopes",
    volume = "70",
    number = "3",
    pages = {483 -- 488},
    year = "2012",
    issn = "0969-8043",
    doi = "10.1016/j.apradiso.2011.11.042",
    author = "Luka Snoj and Gašper Žerovnik and Andrej Trkov",
    keywords = "Research reactor, TRIGA, Irradiation channels, Neutron flux and spectrum"
}

@Article{eudet,
    author="Jansen, Hendrik and others",
    title="Performance of the {EUDET}-type beam telescopes",
    journal="EPJ Techniques and Instrumentation",
    year="2016",
    month="Oct",
    day="04",
    volume="3",
    number="1",
    pages="7",
    abstract="Test beam measurements at the test beam facilities of DESY have been conducted to characterise the performance of the EUDET-type beam telescopes originally developed within the EUDET project. The beam telescopes are equipped with six sensor planes using MIMOSA 26 monolithic active pixel devices. A programmable Trigger Logic Unit provides trigger logic and time stamp information on particle passage. Both data acquisition framework and offline reconstruction software packages are available. User devices are easily integrable into the data acquisition framework via predefined interfaces.",
    issn="2195-7045",
    doi="10.1140/epjti/s40485-016-0033-2",
}

@thesis{pascal:thesis,
    author = {Pascal Wolf},
    title = {Testing and extending a {Python}-based readout system for a high-resolution pixel detector telescope},
    type = {Bachelor Thesis},
    institution = {University of Bonn},
    year = "2016",
}



@article{atlas:pixel,
    author={G Aad and others},
    title={{ATLAS} pixel detector electronics and sensors},
    journal={JINST},
    volume={3},
    number={07},
    pages={P07007},
    url={http://stacks.iop.org/1748-0221/3/i=07/a=P07007},
    year={2008},
    abstract={The silicon pixel tracking system for the ATLAS experiment at the Large Hadron Collider is described and the performance requirements are summarized. Detailed descriptions of the pixel detector electronics and the silicon sensors are given. The design, fabrication, assembly and performance of the pixel detector modules are presented. Data obtained from test beams as well as studies using cosmic rays are also discussed.}
}

@article{fei3,
    title = "The {FEI3} readout chip for the {ATLAS} pixel detector",
    journal = "NIMA",
    volume = "565",
    number = "1",
    pages = {178 -- 187},
    year = "2006",
    issn = "0168-9002",
    doi = "10.1016/j.nima.2006.05.032",
    author = "Ivan Peric and others",
    keywords = "Pixel readout chip, Front end chip, FEI3, ATLAS pixel detector, Radiation tolerant design"
}

@article{fei4,
    title = "The {FE-I4} pixel readout integrated circuit",
    journal = {NIMA},
    volume = "636",
    number = "1, Supplement ",
    pages = {S155 -- S159},
    year = "2011",
    issn = "0168-9002",
    doi = "10.1016/j.nima.2010.04.101",
    author = "M. Garcia-Sciveres and others",
    keywords = "Pixel detector, ATLAS upgrades, High luminosity, 130nm"
}

@online{lf,
    title = {LFoundry},
    url = {http://www.lfoundry.com/},
}

@article{Liu:2017,
    author={J. Liu and others},
    title={Simulations of depleted {CMOS} sensors for high-radiation environments},
    journal={JINST},
    volume={12},
    number={11},
    pages={C11013},
    year={2017},
    abstract={After the Phase II upgrade for the Large Hadron Collider (LHC), the increased luminosity requests a new upgraded Inner Tracker (ITk) for the ATLAS experiment. As a possible option for the ATLAS ITk, a new pixel detector based on High Voltage/High Resistivity CMOS (HV/HR CMOS) technology is under study. Meanwhile, a new CMOS pixel sensor is also under development for the tracker of Circular Electron Position Collider (CEPC). In order to explore the sensor electric properties, such as the breakdown voltage and charge collection efficiency, 2D/3D Technology Computer Aided Design (TCAD) simulations have been performed carefully for the above mentioned both of prototypes. In this paper, the guard-ring simulation for a HV/HR CMOS sensor developed for the ATLAS ITk and the charge collection efficiency simulation for a CMOS sensor explored for the CEPC tracker will be discussed in details. Some comparisons between the simulations and the latest measurements will also be addressed.}
}


@article{Ristic:2015,
    author={B. Ristic},
    title={Measurements on {HV-CMOS} active sensors after irradiation to {HL-LHC} fluences},
    journal={JINST},
    volume={10},
    number={04},
    pages={C04007},
    year={2015},
    abstract={During the long shutdown (LS) 3 beginning 2022 the LHC will be upgraded for higher luminosities pushing the limits especially for the inner tracking detectors of the LHC experiments. In order to cope with the increased particle rate and radiation levels the ATLAS Inner Detector will be completely replaced by a purely silicon based one. Novel sensors based on HV-CMOS processes prove to be good candidates in terms of spatial resolution and radiation hardness. In this paper measurements conducted on prototypes built in the AMS H18 HV-CMOS process and irradiated to fluences of up to 2·10 16 n eq cm −2 are presented.}
}




\bibitem{Lindstrom:2015}
G. Lindstr\"om et al., Radiation hardness of silicon detectors - a challenge from high-energy physics, Nucl. Instr. and Meth. A 246 (1999) 1-15.

\bibitem{Knoll:2015}
G.F. Knoll, Radiation detection and measurements, John Willey and Sons, Inc., New York (2000).

\bibitem{Grupen:2008}
C.G. Grupen and B. Shwartz, Particle Detectors, Cambridge University Press, Cambridge (2008).

\bibitem{lf:2015}
http://www.lfoundry.com/

\bibitem{fei4:2008}
M. Karagounis, Development of the ATLAS FE-I4 pixel readout IC for b-layer Upgrade and Super-LHC, Topical Workshop on Electronics for Particle Physics, Naxos, Greece, 15 - 19 Sep 2008, CERN-2008-008 (2008) 70–75.

\bibitem{elsa:2015}
W. Hillert, The Bonn Electron Stretcher Accelerator ELSA: Past and future, Europ. Phys. Jour. A 28 (2006) 139.

\bibitem{landau:2015}
K. K\"olbig and B. Schorr, A program package for the Landau distribution, Comput. Phys. Commun. 31 (1984) 97-111.

\bibitem{pylandau:2015}
https://pypi.python.org/pypi/pyLandau

\bibitem{Meroll:2015}
S. Meroll et al., Energy loss measurement for charged particle in very thin silicon layers, JINST 6 (2011) P06013.


